Averages of $b$-hadron, $c$-hadron, and $\tau$-lepton properties as of summer 2014

This article reports world averages of measurements of $b$-hadron, $c$-hadron, and $\tau$-lepton properties obtained by the Heavy Flavor Averaging Group (HFAG) using results available through summer 2014. For the averaging, common input parameters used in the various analyses are adjusted (rescaled) to common values, and known correlations are taken into account. The averages include branching fractions, lifetimes, neutral meson mixing parameters, $CP$ violation parameters, parameters of semileptonic decays and CKM matrix elements.

==> b2charm/Bu_cc_7.tex <==
\begin{btocharmtab}{Bu_cc_7}{Direct CP violation parameters}
\hline
\textbf{Parameter} & \begin{tabular}{l}\textbf{Measurements}\end{tabular} & \textbf{Average} \\
\hline
\hline
$A_\mathrm{CP} ( B^- \to J/\psi(1S) K^- )$ & \begin{tabular}{l} \dzero \cite{Abazov:2013sqa}: $0.0059 \pm 0.0036 \pm 0.0007$ \\ \end{tabular} & $0.0059 \pm 0.0037$ \\
\hline
$A_\mathrm{CP} ( B^- \to J/\psi(1S) \pi^- )$ & \begin{tabular}{l} \dzero \cite{Abazov:2013sqa}: $-0.042 \pm 0.044 \pm 0.009$ \\ \end{tabular} & $-0.042 \pm 0.045$ \\
\hline
\end{btocharmtab}


==> hfag_refs.tex <==
% Obsolete 
% \begin{thebibliography}{999}
% 
% %-- Introduction
% 
% \bibitem{ref_ckm}
%  N. Cabibbo, Phys. Rev. Lett. 10, 531 (1963);
%  M. Kobayashi and T. Maskawa, Prog. Theor. Phys. {\bf 49}, 652 (1973).
% 
% \bibitem{LEPHFS}
% ALEPH, CDF, DELPHI, L3, OPAL, 
% and SLD collaborations, ``Combined results on \b-hadron 
% production rates and decay properties'',
% CERN-EP-2000-096, hep-ex/0009052 (2000); updated in
% CERN-EP-2001-050, hep-ex/0112028 (2001).
% 
% \bibitem{PDG_2007}
% W.-M. Yao et al., Journal of Physics, G 33, 1 (2006);
% see also 2007 update at {\tt http://pdg.lbl.gov/}.
% 
% \bibitem{hfag_hepex_endof2006}
%  Heavy Flavor Averaging Group (HFAG), ``Averages of $b$-hadron Properties
%  at the End of 2006'' arXiv:0704.3575 (2007).
% 
% %\bibitem{hfag_hepex_winter2005}
% 
% %\bibitem{Eidelman:2004wy}
% % S.~Eidelman {\em et al.}  (Particle Data Group Collaboration),
% % Phys.\ Lett.\ B {\bf 592}, 1 (2004).
% %%CITATION = PHLTA,B592,1;%%
% 
% %\input{life_mix_references.tex}
% 
% %\input{./slbdecays/slb_refs.tex}
% 
% %\input{cp_uta_refs.tex}
% 
% \input{rare/rare_refs.tex}
% 
% %\input{./charm/charm_refs.tex}
% 
% % \end{thebibliography}


==> tables/cp_uta/psiphi.tex <==
\begin{table}[htb]
	\begin{center}
		\caption{
			 Results from time-dependent analysis of $\Bs \to J/\psi \phi$.
		}
		\vspace{0.2cm}
		\setlength{\tabcolsep}{0.0pc}
% make this tabular (not tabular*) and resize down to \textwidth
% change @{\extracolsep{\fill}} to @{\extracolsep{2mm}}
    \resizebox{\textwidth}{!}{
      \begin{tabular}{@{\extracolsep{2mm}}lrccccc} 
        \hline
        \mc{2}{l}{Experiment} & $\tau(\Bs)$ & $\Delta\Gamma$ & $\phi_s$ & $A_\perp$ & $|A_0|^2 - |A|_\parallel^2$ \\
	\dzero & \cite{:2008fj} & $1.52 \pm 0.06 \pm 0.01$ & $0.19 \pm 0.07 \,^{+0.02}_{-0.01}$ & $-0.57 \,^{+0.24}_{-0.30} \,^{+0.07}_{-0.02}$ & $0.41 \pm 0.04 \,^{+0.01}_{-0.02}$ & $0.34 \pm 0.05 \pm 0.03$ \\
        \hline
      \end{tabular}
    }

		\label{tab:cp_uta:ccs:psiphi}
	\end{center}
\end{table}




==> tau/tau-br-fit-meas-byref.tex <==
%% ///////////////////////////////////////////////////////////////////////////
%%\appendix
\tausection{Branching Fractions Fit Measurement List by Reference}
\cutname{br-fit-meas-byref.html}

Table~\ref{tab:tau:measPerPaper} reports the measurements used for the
\hfagtau branching fraction fit grouped by their bibliographic reference.

%%
%% By-reference measurements list
%%
\begin{center}
\begin{envsmall}
\renewcommand*{\arraystretch}{1.3}%
\ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
\begin{longtable}{ll}
\caption{By-reference measurements list.\label{tab:tau:measPerPaper}}%
\\
\hline
\multicolumn{1}{l}{\bfseries Reference / Branching Fraction} & \multicolumn{1}{l}{\bfseries Value} \\
\hline
\endfirsthead
\multicolumn{2}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \hline
\multicolumn{1}{l}{\bfseries Reference / Branching Fraction} & \multicolumn{1}{l}{\bfseries Value} \\
\hline
\endhead
\htuse{MeasPaper} \\
\hline
\end{longtable}
\end{envsmall}
\end{center}

